Gnuastro: simulating the exposure map of a pointing pattern

The pointing pattern is an integral part of designing one's observation strategy for a certain scientific goal. But accounting for the particular science case or instrument artifacts (like distortion, vignetting or large areas of bad pixels) can make it hard to predict how the exposure map of the final stack will be. To help address this problem, Gnuastro 0.21 includes a new executable program called astscript-pointing-simulate that is fully described in the Gnuastro manual and comes with a complete tutorial. The figures of this research note are reproducible with Maneage, on the Git commit 4176d29.

==> project <==
#!/bin/sh
#
# High-level script to manage the project.
# Run './project --help' for a description of how to use it.
#
# Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
# Copyright (C) 2021-2023 Raul Infante-Sainz <infantesainz@gmail.com>
#
# This program is free software: you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation, either version 3 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program.  If not, see <http://www.gnu.org/licenses/>.


# Basic settings
# --------------
# Stop the script if there are any errors.
set -e





# Default option values
jobs=0     # 0 is for the default for the 'configure.sh' script.
group=
debug=
host_cc=0
operation=
build_dir=
input_dir=
check_config=
make_targets=
software_dir=
clean_texdir=0
prepare_redo=0
highlightnew=0
all_highlevel=0
existing_conf=0
highlightnotes=0
scriptname="./project"





# Parse the options
# -----------------
#
# Separate command-line arguments from options. Then put the option value
# into the respective variable.
#
# Each option has two lines because we want to process both these formats:
# '--name=value' and '--name value'. The former (with '=') is a single
# command-line argument, so we just need to shift the counter by one. The
# latter (without '=') is two arguments, so we'll need two shifts.
#
# Note on the case strings: for every option, we need three lines: one when
# the option name and value are separate. Another when there is an equal
# between them, and finally one where the value is immediately after the
# short-format. This exact order is important. Otherwise, there will be a
# conflict between them.

print_help() {
    # Print the output.
    cat <<EOF
Usage: $scriptname configure [OPTIONS]
       $scriptname shell     [OPTIONS]
       $scriptname make      [OPTIONS]

Top-level script to manage the reproducible project. The high-level
operation is defined by the (mandatory) second argument:

  configure    - Configure project for this machine (e.g., build software).
  make         - Run the project (do analysis and build outputs).
  shell        - Execute the project's shell for interactive testing.

RECOMMENDATION: If this is the first time you are configuring this
template, please don't use the options and let the script explain each
parameter in full detail by simply running './project configure'.

Project 'make' special features.
  ./project make           Build the project on one thread
  ./project make -jN       Built the project in parallel on N threads.
  ./project make clean     Clean all files generated by 'make' (not software).
  ./project make texclean  Clean all files built by (La)TeX.
  ./project make distclean Clean everything (including compiled software).
  ./project make dist      Produce a LaTeX-ready-to-build distribution tarball
                           ('tar.gz') of the project. This is ready to be
                           uploaded to servers like 'arXiv.org'.
  ./project make dist-singledir-onlypaper: in the build/analysis directory.
  ./project make dist-lzip Similar to 'dist', but compress to '.tar.lz'.
  ./project make dist-zip  Similar to 'dist', but compress to '.zip'.
  ./project make dist-software  Build a .tar.gz tarball containing all
                                software source tarballs necessary for the
                                project.

With the options below you can modify the default behavior.
Configure options:
  -b, --build-dir=STR      Top directory to build the project in.
  -e, --existing-conf      Use (possibly existing) local configuration.
      --host-cc            Use host system's C compiler, don't build GCC.
  -i, --input-dir=STR      Directory containing input datasets (optional).
  -s, --software-dir=STR   Directory containing necessary software tarballs.
      --check-config       During configuration, show what is being built.
      --clean-texdir       Remove possibly existing build-time subdirectories
                           under the project's 'tex/' directory (can happen
                           when source is from arXiv for example).
      --all-highlevel      Build all high-level software (for development).

Configure and Make options:
  -d, --debug[=FLAGS]      In configure: use -j1, no -k, and no Zenodo check.
                           In make: 'FLAGS' will be directly passed to 'make'.
  -g, --group=STR          Build and run with write permissions for a group.
  -j, --jobs=INT           Number of threads to build/run the software.
  -?, --help               Print this help list.

Make (analysis) options:
  -p, --prepare-redo       Re-do preparation (only done automatically once).

Make (final PDF) options:
      --refresh-bib        Force refresh the bibliography.
      --highlight-new      Highlight '\new' parts of text as green.
      --highlight-notes    Show '\tonote' regions as red text in PDF.

Mandatory or optional arguments to long options are also mandatory or optional
for any corresponding short options.

Maneage URL: https://maneage.org

Report bugs to mohammad@akhlaghi.org
EOF
}

on_off_option_error() {
    if [ "x$2" = x ]; then
        echo "$scriptname: '$1' doesn't take any values."
    else
        echo "$scriptname: '$1' (or '$2') doesn't take any values."
    fi
    exit 1
}

check_v() {
    if [ x"$2" = x ]; then
        echo "$scriptname: option '$1' requires an argument."
        echo "Try '$scriptname --help' for more information."
        exit 1;
    fi
}

func_operation_set() {
    if [ x$operation = x ]; then
        operation=$1
    else
        echo "Only one operation ('configure', 'make' or 'shell') may be given."
        exit 1
    fi
}

while [ $# -gt 0 ]
do
 case $1 in
  # Main operation.
  configure)    func_operation_set $1; shift;;
  make)         func_operation_set $1; shift;;
  shell)        func_operation_set $1; shift;;

  # Configure options:
  -b|--build-dir)        build_dir="$2";                                     check_v "$1" "$build_dir";    shift;shift;;
  -b=*|--build-dir=*)    build_dir="${1#*=}";                                check_v "$1" "$build_dir";    shift;;
  -b*)                   build_dir=$(echo    "$1" | sed -e's/-b//');         check_v "$1" "$build_dir";    shift;;
  -e|--existing-conf)    existing_conf=1;                                                                  shift;;
  -e*|--existing-conf=*) on_off_option_error --existing-conf -e;;
  --host-cc)             host_cc=1;                                                                        shift;;
  --host-cc=*)           on_off_option_error --host-cc;;
  -i|--input-dir)        input_dir="$2";                                     check_v "$1" "$input_dir";    shift;shift;;
  -i=*|--input-dir=*)    input_dir="${1#*=}";                                check_v "$1" "$input_dir";    shift;;
  -i*)                   input_dir=$(echo    "$1" | sed -e's/-i//');         check_v "$1" "$input_dir";    shift;;
  -s|--software-dir)     software_dir="$2";                                  check_v "$1" "$software_dir"; shift;shift;;
  -s=*|--software-dir=*) software_dir="${1#*=}";                             check_v "$1" "$software_dir"; shift;;
  -s*)                   software_dir=$(echo "$1" | sed -e's/-s//');         check_v "$1" "$software_dir"; shift;;
  --check-config)        check_config=1;                                                                   shift;;
  --check-config=*)      on_off_option_error --check-config;;
  --clean-texdir)        clean_texdir=1;                                                                   shift;;
  --clean-texdir=*)      on_off_option_error --clean-texdir;;
  --all-highlevel)       all_highlevel=1;                                                                  shift;;
  --all-highlevel=*)     on_off_option_error --all-highlevel;;

  # Configure and Make options:
  -g|--group)             group="$2";                            check_v group "$group";   shift;shift;;
  -g=*|--group=*)         group="${1#*=}";                       check_v group "$group";   shift;;
  -g*)                    group=$(echo   "$1" | sed -e's/-g//'); check_v group "$group";   shift;;
  -j|--jobs)              jobs="$2";                             check_v jobs  "$jobs";    shift;shift;;
  -j=*|--jobs=*)          jobs="${1#*=}";                        check_v jobs  "$jobs";    shift;;
  -j*)                    jobs=$(echo "$1" | sed -e's/-j//');    check_v jobs  "$jobs";    shift;;
  -'?'|--help)            print_help; exit 0;;
  -'?'*|--help=*)         on_off_option_error --help -?;;

  # Make options
  # ------------
  #
  # Note that Make's 'debug' can take values, but when called without any
  # value, it is like giving it a value of 'a'):
  --refresh-bib)          [ -f tex/src/references.tex ] && touch tex/src/references.tex;   shift;;
  --highlight-new)        highlightnew=1;                                                  shift;;
  --highlight-new=*)      on_off_option_error --highlight-new;;
  --highlight-notes)      highlightnotes=1;                                                shift;;
  --highlight-notes=*)    on_off_option_error --highlight-notes;;
  -d|--debug)             if [ x$operation = x ]; then
                              echo "Please set the operation before calling '--debug'"; exit 1
                          elif [ x$operation = xconfigure ]; then debug=a;   shift;
                          elif [ x$operation = xmake ]; then
                              if [ x"$2" = x ]; then echo "In make-mode, '--debug' needs a value"; exit 1
                              else debug="$2"; check_v debug "$debug"; shift;shift; fi
                          else
                              echo "Operation '$operation' not recognized, please use 'configure' or 'make'"
                          fi;;
  -d=*|--debug=*)         debug="${1#*=}";                       check_v debug "$debug";   shift;;
  -d*)                    debug=$(echo "$1" | sed -e's/-d//');   check_v debug "$debug";   shift;;
  -p|--prepare-redo)      prepare_redo=1;                                                  shift;;
  -p=*|--prepare-redo=*)  on_off_option_error --prepare-redo;                              shift;;

  # Unrecognized option:
  -*) echo "$scriptname: unknown option '$1'"; exit 1;;

  # Not an option, an argument (so its a Make target).
  *) make_targets="$make_targets $1"; shift;;
 esac
done





# Check configuration status
# --------------------------
if ! [ x$check_config = x ]; then
    # Find the color option to pass to 'ls'. Note that '--color' (for GNU
    # Coreutils 'ls') should be checked first because it also has '-G', but
    # for something else.
    if   ls --color 2> /dev/null > /dev/null; then coloropt="--color=auto"
    elif ls -G      2> /dev/null > /dev/null; then coloropt="-G"
    else                               coloropt=""
    fi

    # Print a notice to let the user know what is happening.
    cat <<EOF

This is an infinite loop that will print what software are being built at
every moment. It is actually a listing ('ls' command) of the temporary
directory where software source code are unpacked while they are being
built. If the project isn't being configured, the output (every second)
will either be empty (only a date) or a with an error about a non-existant
directory. This feature is thus only useful when the project's software are
being built.

EOF

    # Run the infinite loop. To be able to find the last built programs, we
    # need to put all the Python programs and high-level program into one
    # directory.
    checkdir=.local/version-info/.for-check-config
    while true; do

        # Make sure the '.build' directory has already been created.
        echo;
        echo "========================"
        if [ -d .build ]; then
            echo "$(date)    [[press CTRL-C to stop]]";
            echo "--- Currently being built:"
            if [ -d .build/software/build-tmp ]; then
                ls $coloropt .build/software/build-tmp || junk=1;
            fi

            # Make the temporary directory, delete its contents, then put new
            # links of all built software.
            if ! [ -d $checkdir ]; then mkdir $checkdir; fi
            rm -f $checkdir/*

            # Check if any programs exist in the given directory yet.
            printresults=0
            check=$(ls .local/version-info/python/)
            if ! [ "x$check" = x ]; then
                printresults=1
                ln -s "$(pwd)"/.local/version-info/python/*  $checkdir/
            fi
            check=$(ls .local/version-info/proglib/)
            if ! [ "x$check" = x ]; then
                printresults=1
                ln -s "$(pwd)"/.local/version-info/proglib/* $checkdir/
            fi

            # If something was actually found, then print them.
            if [ $printresults = 1 ]; then
                echo "--- Last 5 packages that were built:"

                # Then sort all the links based on the most recent dates of the
                # files they link to (with '-L').
                ls -Llt $checkdir  \
                    | awk '/^-/ && c++<5 {printf "[at %s] %s\n", $(NF-1), $NF}'
            fi
        else
            cat <<EOF
The connection to the build directory (.build) is not yet created.

If you have just ran './project configure', it should be created and will
be used in a few seconds to report the build status of various software.
If not, please run './project configure' (in another terminal) and you will
see the results shortly afterwards.
EOF
        fi
        echo "========================"

        # Wait for the next round of checks.
        sleep 1
    done
    exit 0
fi





# Basic group settings
# --------------------
if ! [ x$group = x ]; then

    # Check if group is usable.
    if ! sg "$group" "echo Group \'$group\' exists"; then
        echo "$scriptname: '$group' is not a usable group name on this system.";
        echo "(TIP: you can use the 'groups' command to see your groups)"
        exit 1
    fi

    # Set the group option for running Make.
    gopt="maneage_group_name=$group"
fi





# Error when configuration isn't run
configuration_necessary() {
    cat <<EOF

The project is either (1) not configured on this system, or (2) the
configuration wasn't successful.

(1) If it hasn't been configured at all, use the command below to configure
it (set a build directory and let it build its necessary software in it).

      $ ./project configure

(2) If it has been configured, but the configuration failed in a step, you
can re-configure it using your previous settings with the command
below. All successful steps will be skipped, allowing a fast completion.

      $ ./project configure -e

If there was a problem, please let us know by filling this online form:
      http://savannah.nongnu.org/support/?func=additem&group=reproduce

EOF
    exit 1
}





# Run operations in controlled environment
# ----------------------------------------
controlled_env() {

    # Get the full address of the build directory:
    bdir=`.local/bin/realpath .build`

    # Remove all existing environment variables (with 'env -i') and only
    # use some pre-defined environment variables, then build the project.
    envmake=".local/bin/env -i HOME=$bdir sys_rm=$(which rm) $gopt"
    envmake="$envmake highlightnew=$highlightnew"
    envmake="$envmake highlightnotes=$highlightnotes .local/bin/make"
    envmake="$envmake --no-builtin-rules --no-builtin-variables -f $1"
    if ! [ x"$debug" = x  ]; then envmake="$envmake --debug=$debug"; fi

    # Set the number of jobs. Note that for the 'configure.sh' script the
    # default value has to be 0, so the default is the maximum number of
    # threads. But here, the default value is 1.
    if ! [ x"$jobs"  = x0 ]; then envmake="$envmake -j$jobs";  fi

    # Run the project
    if [ x"$group" = x ]; then
        $envmake $make_targets
    else
        # Set the group and permission flags.
        sg "$group" "umask $perms && $envmake $make_targets"
    fi
}





# Do requested operation
# ----------------------
perms="u+r,u+w,g+r,g+w,o-r,o-w,o-x"
configscript=./reproduce/software/shell/configure.sh
case $operation in

    # Build the project's software.
    configure)

        # Set executable flags
        # --------------------
        #
        # In some scenarios (for example when using a tarball from arXiv),
        # it may happen that the host server has removed the executable
        # flags of all the files. In 'README.md' we instruct the readers on
        # setting the executable flag of this script. But we don't want the
        # user to have to worry about any other file that needs an
        # executable flag.
        #
        # Basically, all the project shell scripts need executable flags so
        # to make sure they have them, we are activating the executable
        # flags by default here every time './project configure' is run. If
        # any other file in your project needs such flags, add them here.
        chmod +x reproduce/software/shell/* reproduce/software/config/*.sh \
              reproduce/analysis/bash/*

        # If the user requested, clean the TeX directory from the extra
        # (to-be-built) directories that may already be there (and will not
        # allow the configuration to complete).
        if [ x"$clean_texdir" = x1 ]; then
            rm -rf tex/build tex/tikz
        fi

        # Variables to pass to the configuration script.
        export jobs=$jobs
        export debug=$debug
        export host_cc=$host_cc
        export build_dir=$build_dir
        export input_dir=$input_dir
        export scriptname=$scriptname
        export maneage_group_name=$group
        export software_dir=$software_dir
        export existing_conf=$existing_conf
        export all_highlevel=$all_highlevel

        # Run the configuration script
        if [ x"$group" = x ]; then
            $configscript
        else
            # Set the group and permission flags.
            sg "$group" "umask $perms && $configscript"

            # Set the group writing permission for everything in the
            # installed software directory. The common build process sets
            # the writing permissions of the installed programs/libraries
            # to '755'. So group members can't write over a file. This
            # creates problems when another group member wants to update
            # the software for example. We thus need to manually add the
            # group writing flag to all installed software files.
            echo "Enabling group writing permission on all installed software..."
            .local/bin/chmod -R g+w .local/;
        fi
        ;;





    # Batch execution of the project.
    make)

        # Make sure the configure script has been completed properly
        # ('configuration-done.txt' exists).
        if ! [ -f .build/software/configuration-done.txt ]; then
            configuration_necessary
        fi

        # Run data preparation phase (optionally build Makefiles with
        # special values for optimizing the main 'top-make.mk'). But note
        # that data preparation is only done automatically the first time
        # the project is built (when '.build/software/preparation-done.mk'
        # doesn't yet exist). After that, if the user wants to re-do the
        # preparation they have to use the '--prepare-redo' option.
        if ! [ -f .build/software/preparation-done.mk ] \
                || [ x"$prepare_redo" = x1 ]; then
            controlled_env reproduce/analysis/make/top-prepare.mk
        fi

        # Run the actual project.
        controlled_env reproduce/analysis/make/top-make.mk
        ;;


    shell)

        # Make sure the configure script has been completed properly
        # ('configuration-done.txt' exists).
        if ! [ -f .build/software/configuration-done.txt ]; then
            configuration_necessary
        fi

        # Run the project's own shell without inheriting any environment
        # from the host. The 'TERM' environment variable is necessary for
        # tools like some text editors.
        bdir=`.local/bin/realpath .build`
        instdir="$bdir"/software/installed
        bindir="$bdir"/software/installed/bin
        rcfile=$(pwd)/reproduce/software/shell/bashrc.sh
        .local/bin/env -i \
                       HOME="$bdir" \
                       TERM="$TERM" \
                       PATH="$bindir" \
                       CCACHE_DISABLE=1 \
                       PROJECT_STATUS=shell \
                       SHELL="$bindir"/bash \
                       COLORTERM="$COLORTERM" \
                       PROJECT_RCFILE="$rcfile" \
                       LDFLAGS=-L"$instdir"/lib \
                       CPPFLAGS=-I"$instdir"/include \
                       LD_LIBRARY_PATH="$instdir"/lib \
                       OMPI_MCA_plm_rsh_agent=/bin/false \
                       PYTHONPATH="$instdir"/lib/python/site-packages \
                       PYTHONPATH3="$instdir"/lib/python/site-packages \
                       PS1="[\[\033[01;35m\]maneage@\h \W\[\033[32m\]\[\033[00m\]]$ " \
                       "$bindir"/bash --noprofile --rcfile "$rcfile"
        ;;


    # Operation not specified.
    *)
        cat <<EOF

No operation defined!

Please run with '--help' for more information.
(TIP: available operations are: 'configure', 'make', or 'shell').

EOF
        exit 1
        ;;
esac


==> reproduce/analysis/bash/download-multi-try <==
#!/bin/sh
#
# Attempt downloading multiple times before crashing whole project. From
# the top project directory (for the shebang above), this script must be
# run like this:
#
#   $ /path/to/download-multi-try downloader lockfile input-url downloaded-name
#
# NOTE: The 'downloader' must contain the option to specify the output name
# in its end. For example "wget -O". Any other option can also be placed in
# the middle.
#
# Due to temporary network problems, a download may fail suddenly, but
# succeed in a second try a few seconds later. Without this script that
# temporary glitch in the network will permanently crash the project and
# it can't continue. The job of this script is to be patient and try the
# download multiple times before crashing the whole project.
#
# LOCK FILE: Since there is usually only one network port to the outside
# world, downloading is done much faster in serial, not in parallel. But
# the project's processing may be done in parallel (with multiple threads
# needing to download different files at the same time). Therefore, this
# script uses the 'flock' program to only do one download at a time. To
# benefit from it, any call to this script must be given the same lock
# file. If your system has multiple ports to the internet, or for any
# reason, you don't want to use a lock file, set the 'lockfile' name to
# 'nolock'.
#
# Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# This program is free software: you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation, either version 3 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program.  If not, see <http://www.gnu.org/licenses/>.





# Script settings
# ---------------
# Stop the script if there are any errors.
set -e





# Input arguments and necessary sanity checks. Note that the 5th argument
# (backup servers) isn't mandatory.
inurl="$3"
outname="$4"
lockfile="$2"
downloader="$1"
backupservers="$5"
if [ "x$downloader" = x ]; then
    echo "$0: downloader (first argument) not given."; exit 1;
fi
if [ "x$lockfile" = x ]; then
    echo "$0: lock file (second argument) not given."; exit 1;
fi
if [ "x$inurl" = x ]; then
    echo "$0: full input URL (third argument) not given."; exit 1;
fi
if [ "x$outname" = x ]; then
    echo "$0: output name (fourth argument) not given."; exit 1;
fi





# Separate the actual filename, to possibly use backup server.
urlfile=$(echo "$inurl" | awk -F "/" '{print $NF}')





# Try downloading multiple times before crashing.
counter=0
maxcounter=10
while [ ! -f "$outname" ]; do

    # Increment the counter.
    counter=$(echo $counter | awk '{print $1+1}')

    # If we have passed a maximum number of trials, just exit with
    # a failed code.
    reachedmax=$(echo $counter \
         | awk '{if($1>'$maxcounter') print "yes"; else print "no";}')
    if [ x$reachedmax = xyes ]; then
        echo ""
	echo "Failed $maxcounter download attempts: $outname"
        echo ""
	exit 1
    fi

    # If this isn't the first attempt print a notice and wait a little for
    # the next trail.
    if [ x$counter = x1 ]; then
        just_a_place_holder=1
    else
        tstep=$(echo $counter | awk '{print $1*5}')
        echo "Download trial $counter for '$outname' in $tstep seconds."
        sleep $tstep
    fi

    # Attempt downloading the file. Note that the 'downloader' ends with
    # the respective option to specify the output name. For example "wget
    # -O" (so 'outname', that comes after it) will be the name of the
    # downloaded file.
    if [ x"$lockfile" = xnolock ]; then
        if ! $downloader $outname $inurl; then rm -f $outname; fi
    else
        # Try downloading from the requested URL.
        flock "$lockfile" sh -c \
              "if ! $downloader $outname \"$inurl\"; then rm -f $outname; fi"
    fi

    # If the download failed, try the backup server(s).
    if [ ! -f "$outname" ]; then
        if [ x"$backupservers" != x ]; then
            for bs in $backupservers; do

                # Use this backup server.
                if [ x"$lockfile" = xnolock ]; then
                    if ! $downloader $outname $bs/$urlfile; then rm -f $outname; fi
                else
                    flock "$lockfile" sh -c \
                          "if ! $downloader $outname $bs/$urlfile; then rm -f $outname; fi"
                fi

                # If the file was downloaded, break out of the loop that
                # parses over the backup servers.
                if [ -f "$outname" ]; then break; fi
            done
        fi
    fi
done





# Return successfully
exit 0


==> reproduce/software/bibtex/astrometrynet.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{astrometrynet,
       author = {{Lang}, Dustin and {Hogg}, David W. and {Mierle}, Keir and {Blanton}, Michael and {Roweis}, Sam},
        title = "{Astrometry.net: Blind Astrometric Calibration of Arbitrary Astronomical Images}",
      journal = {AJ},
     keywords = {astrometry, catalogs, instrumentation: miscellaneous, methods: data analysis, methods: statistical, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2010,
        month = may,
       volume = {139},
       number = {5},
        pages = {1782-1800},
          doi = {10.1088/0004-6256/139/5/1782},
archivePrefix = {arXiv},
       eprint = {0910.2233},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010AJ....139.1782L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/astropy.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{astropy2018,
   author = {{Astropy Collaboration} and {Price-Whelan}, A.~M. and {Sip{\H o}cz}, B.~M. and
	{G{\"u}nther}, H.~M. and {Lim}, P.~L. and {Crawford}, S.~M. and
	{Conseil}, S. and {Shupe}, D.~L. and {Craig}, M.~W. and {Dencheva}, N. and
	{Ginsburg}, A. and {VanderPlas}, J.~T. and {Bradley}, L.~D. and
	{P{\'e}rez-Su{\'a}rez}, D. and {de Val-Borro}, M. and {Aldcroft}, T.~L. and
	{Cruz}, K.~L. and {Robitaille}, T.~P. and {Tollerud}, E.~J. and
	{Ardelean}, C. and {Babej}, T. and {Bach}, Y.~P. and {Bachetti}, M. and
	{Bakanov}, A.~V. and {Bamford}, S.~P. and {Barentsen}, G. and
	{Barmby}, P. and {Baumbach}, A. and {Berry}, K.~L. and {Biscani}, F. and
	{Boquien}, M. and {Bostroem}, K.~A. and {Bouma}, L.~G. and {Brammer}, G.~B. and
	{Bray}, E.~M. and {Breytenbach}, H. and {Buddelmeijer}, H. and
	{Burke}, D.~J. and {Calderone}, G. and {Cano Rodr{\'{\i}}guez}, J.~L. and
	{Cara}, M. and {Cardoso}, J.~V.~M. and {Cheedella}, S. and {Copin}, Y. and
	{Corrales}, L. and {Crichton}, D. and {D'Avella}, D. and {Deil}, C. and
	{Depagne}, {\'E}. and {Dietrich}, J.~P. and {Donath}, A. and
	{Droettboom}, M. and {Earl}, N. and {Erben}, T. and {Fabbro}, S. and
	{Ferreira}, L.~A. and {Finethy}, T. and {Fox}, R.~T. and {Garrison}, L.~H. and
	{Gibbons}, S.~L.~J. and {Goldstein}, D.~A. and {Gommers}, R. and
	{Greco}, J.~P. and {Greenfield}, P. and {Groener}, A.~M. and
	{Grollier}, F. and {Hagen}, A. and {Hirst}, P. and {Homeier}, D. and
	{Horton}, A.~J. and {Hosseinzadeh}, G. and {Hu}, L. and {Hunkeler}, J.~S. and
	{Ivezi{\'c}}, {\v Z}. and {Jain}, A. and {Jenness}, T. and {Kanarek}, G. and
	{Kendrew}, S. and {Kern}, N.~S. and {Kerzendorf}, W.~E. and
	{Khvalko}, A. and {King}, J. and {Kirkby}, D. and {Kulkarni}, A.~M. and
	{Kumar}, A. and {Lee}, A. and {Lenz}, D. and {Littlefair}, S.~P. and
	{Ma}, Z. and {Macleod}, D.~M. and {Mastropietro}, M. and {McCully}, C. and
	{Montagnac}, S. and {Morris}, B.~M. and {Mueller}, M. and {Mumford}, S.~J. and
	{Muna}, D. and {Murphy}, N.~A. and {Nelson}, S. and {Nguyen}, G.~H. and
	{Ninan}, J.~P. and {N{\"o}the}, M. and {Ogaz}, S. and {Oh}, S. and
	{Parejko}, J.~K. and {Parley}, N. and {Pascual}, S. and {Patil}, R. and
	{Patil}, A.~A. and {Plunkett}, A.~L. and {Prochaska}, J.~X. and
	{Rastogi}, T. and {Reddy Janga}, V. and {Sabater}, J. and {Sakurikar}, P. and
	{Seifert}, M. and {Sherbert}, L.~E. and {Sherwood-Taylor}, H. and
	{Shih}, A.~Y. and {Sick}, J. and {Silbiger}, M.~T. and {Singanamalla}, S. and
	{Singer}, L.~P. and {Sladen}, P.~H. and {Sooley}, K.~A. and
	{Sornarajah}, S. and {Streicher}, O. and {Teuben}, P. and {Thomas}, S.~W. and
	{Tremblay}, G.~R. and {Turner}, J.~E.~H. and {Terr{\'o}n}, V. and
	{van Kerkwijk}, M.~H. and {de la Vega}, A. and {Watkins}, L.~L. and
	{Weaver}, B.~A. and {Whitmore}, J.~B. and {Woillez}, J. and
	{Zabalza}, V. and {Astropy Contributors}},
    title = "{The Astropy Project: Building an Open-science Project and Status of the v2.0 Core Package}",
  journal = {AJ},
archivePrefix = "arXiv",
   eprint = {1801.02634},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, methods: statistical, reference systems },
     year = 2018,
    month = sep,
   volume = 156,
      eid = {123},
    pages = {123},
      doi = {10.3847/1538-3881/aabc4f},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..123A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{astropy2013,
   author = {{Astropy Collaboration} and {Robitaille}, T.~P. and {Tollerud}, E.~J. and
	{Greenfield}, P. and {Droettboom}, M. and {Bray}, E. and {Aldcroft}, T. and
	{Davis}, M. and {Ginsburg}, A. and {Price-Whelan}, A.~M. and
	{Kerzendorf}, W.~E. and {Conley}, A. and {Crighton}, N. and
	{Barbary}, K. and {Muna}, D. and {Ferguson}, H. and {Grollier}, F. and
	{Parikh}, M.~M. and {Nair}, P.~H. and {Unther}, H.~M. and {Deil}, C. and
	{Woillez}, J. and {Conseil}, S. and {Kramer}, R. and {Turner}, J.~E.~H. and
	{Singer}, L. and {Fox}, R. and {Weaver}, B.~A. and {Zabalza}, V. and
	{Edwards}, Z.~I. and {Azalee Bostroem}, K. and {Burke}, D.~J. and
	{Casey}, A.~R. and {Crawford}, S.~M. and {Dencheva}, N. and
	{Ely}, J. and {Jenness}, T. and {Labrie}, K. and {Lim}, P.~L. and
	{Pierfederici}, F. and {Pontzen}, A. and {Ptak}, A. and {Refsdal}, B. and
	{Servillat}, M. and {Streicher}, O.},
    title = "{Astropy: A community Python package for astronomy}",
  journal = {A\&A},
archivePrefix = "arXiv",
   eprint = {1307.6212},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {A33},
    pages = {A33},
      doi = {10.1051/0004-6361/201322068},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2013A\%26A...558A..33A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/corner.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{corner,
       author = {{Foreman-Mackey}, Daniel},
        title = "{corner.py: Scatterplot matrices in Python}",
      journal = {JOSS},
         year = "2016",
        month = "Jun",
       volume = {1},
        pages = {24},
          doi = {10.21105/joss.00024},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016JOSS....1...24F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/cython.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{cython2011,
       author = {{Behnel}, Stefan and {Bradshaw}, Robert and {Citro}, Craig and {Dalcin}, Lisandro and {Seljebotn}, Dag Sverre and {Smith}, Kurt},
        title = "{Cython: The Best of Both Worlds}",
      journal = {Computing in Science and Engineering},
         year = 2011,
        month = mar,
       volume = {13},
       number = {2},
        pages = {31-39},
          doi = {10.1109/MCSE.2010.118},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011CSE....13b..31B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/fftw.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{fftw,
   author = {M. {Frigo} and S. G. {Johnson}},
  journal = {IEEE Proc.},
    title = {The Design and Implementation of FFTW3},
     year = {2005},
   volume = {93},
   number = {2},
    pages = {216-231},
      doi = {10.1109/JPROC.2004.840301},
     ISSN = {0018-9219},
    month = {Feb},
}


==> reproduce/software/bibtex/galsim.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{galsim,
       author = {{Rowe}, B.~T.~P. and {Jarvis}, M. and {Mandelbaum}, R. and
         {Bernstein}, G.~M. and {Bosch}, J. and {Simet}, M. and {Meyers}, J.~E. and
         {Kacprzak}, T. and {Nakajima}, R. and {Zuntz}, J. and {Miyatake}, H. and
         {Dietrich}, J.~P. and {Armstrong}, R. and {Melchior}, P. and
         {Gill}, M.~S.~S.},
        title = "{GALSIM: The modular galaxy image simulation toolkit}",
      journal = {Astron.Comput.},
     keywords = {Methods: data analysis, Techniques: image processing, Gravitational lensing, Cosmology: observations, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, 85-04},
         year = "2015",
        month = "Apr",
       volume = {10},
        pages = {121-150},
          doi = {10.1016/j.ascom.2015.02.002},
archivePrefix = {arXiv},
       eprint = {1407.7676},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&C....10..121R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/gnuastro.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{gnuastro,
       author = {{Akhlaghi}, Mohammad and {Ichikawa}, Takashi},
        title = "{Noise-based Detection and Segmentation of Nebulous Objects}",
      journal = {ApJS},
     keywords = {galaxies: irregular, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = sep,
       volume = {220},
       number = {1},
          eid = {1},
        pages = {1},
          doi = {10.1088/0067-0049/220/1/1},
archivePrefix = {arXiv},
       eprint = {1505.01664},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..220....1A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/healpix.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{healpix,
       author = {{G{\'o}rski}, K.~M. and {Hivon}, E. and {Banday}, A.~J. and {Wandelt}, B.~D. and {Hansen}, F.~K. and {Reinecke}, M. and {Bartelmann}, M.},
        title = "{HEALPix: A Framework for High-Resolution Discretization and Fast Analysis of Data Distributed on the Sphere}",
      journal = {ApJ},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Observations, Methods: Statistical, Astrophysics},
         year = 2005,
        month = apr,
       volume = {622},
       number = {2},
        pages = {759-771},
          doi = {10.1086/427976},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409513},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...622..759G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/imfit.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{imfit2015,
       author = {{Erwin}, Peter},
        title = "{IMFIT: A Fast, Flexible New Program for Astronomical Image Fitting}",
      journal = {ApJ},
     keywords = {galaxies: bulges, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = feb,
       volume = {799},
       number = {2},
          eid = {226},
        pages = {226},
          doi = {10.1088/0004-637X/799/2/226},
archivePrefix = {arXiv},
       eprint = {1408.1097},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...799..226E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/matplotlib.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{matplotlib2007,
       author = {{Hunter}, John D.},
        title = "{Matplotlib: A 2D Graphics Environment}",
      journal = {CiSE},
     keywords = {Python, Scripting languages, Application development, Scientific programming},
         year = 2007,
        month = may,
       volume = {9},
       number = {3},
        pages = {90-95},
          doi = {10.1109/MCSE.2007.55},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007CSE.....9...90H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/missfits.tex <==
%% Copyright (C) 2020-2023 Surena Fatemi <surena.fatemi@ipm.ir>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{missfits,
       author = {{Marmo}, C. and {Bertin}, E.},
        title = "{MissFITS and WeightWatcher: Two Optimised Tools for Managing FITS Data.}",
      journal = {ASPC},
         year = 2008,
       volume = {394},
       series = {Astronomical Society of the Pacific Conference Series},
        pages = {619},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ASPC..394..619M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/mpi4py.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{mpi4py2011,
       author = {{Dalcin}, Lisandro D. and {Paz}, Rodrigo R. and {Kler}, Pablo A. and {Cosimo}, Alejandro},
        title = "{Parallel distributed computing using Python}",
      journal = {Advances in Water Resources},
         year = 2011,
        month = sep,
       volume = {34},
       number = {9},
        pages = {1124-1139},
          doi = {10.1016/j.advwatres.2011.04.013},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011AdWR...34.1124D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/numpy.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{numpy2020,
       author = {{Harris}, Charles R. and {Millman}, K. Jarrod and {van der Walt}, St{\'e}fan J. and {Gommers}, Ralf and {Virtanen}, Pauli and {Cournapeau}, David and {Wieser}, Eric and {Taylor}, Julian and {Berg}, Sebastian and {Smith}, Nathaniel J. and {Kern}, Robert and {Picus}, Matti and {Hoyer}, Stephan and {van Kerkwijk}, Marten H. and {Brett}, Matthew and {Haldane}, Allan and {del R{\'\i}o}, Jaime Fern{\'a}ndez and {Wiebe}, Mark and {Peterson}, Pearu and {G{\'e}rard-Marchant}, Pierre and {Sheppard}, Kevin and {Reddy}, Tyler and {Weckesser}, Warren and {Abbasi}, Hameer and {Gohlke}, Christoph and {Oliphant}, Travis E.},
        title = "{Array programming with NumPy}",
      journal = {Nature},
     keywords = {Computer Science - Mathematical Software, Statistics - Computation},
         year = 2020,
        month = sep,
       volume = {585},
       number = {7825},
        pages = {357-362},
          doi = {10.1038/s41586-020-2649-2},
archivePrefix = {arXiv},
       eprint = {2006.10256},
 primaryClass = {cs.MS},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020Natur.585..357H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/r-cran.tex <==
%% Copyright (C) 2022-2023 Boud Roukema <boud@cosmo.torun.pl>
%% Copyright (C) 2022-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{RIhakaGentleman1996,
      author = {{Ihaka}, Ross and {Gentleman}, Robert},
       title = "{R: A language for data analysis and graphics}",
     journal = {J.Comput.Graph.Stat.},
        year = {1996},
      volume = {5},
      number = {3},
       pages = {299-314},
         DOI = {10.1080/10618600.1996.10474713},
        ISSN = {10618600},
}


==> reproduce/software/bibtex/scamp.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{scamp,
   author = {{Bertin}, E.},
    title = "{Automatic Astrometric and Photometric Calibration with SCAMP}",
     year = 2006,
   journal= {ASPConf},
   volume = 351,
    month = jul,
    pages = {112},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2006ASPC..351..112B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/scipy.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{scipy2020,
       author = {{Virtanen}, Pauli and {Gommers}, Ralf and {Oliphant}, Travis E. and {Haberland}, Matt and {Reddy}, Tyler and {Cournapeau}, David and {Burovski}, Evgeni and {Peterson}, Pearu and {Weckesser}, Warren and {Bright}, Jonathan and {van der Walt}, St{\'e}fan J. and {Brett}, Matthew and {Wilson}, Joshua and {Millman}, K. Jarrod and {Mayorov}, Nikolay and {Nelson}, Andrew R.~J. and {Jones}, Eric and {Kern}, Robert and {Larson}, Eric and {Carey}, C.~J. and {Polat}, {\.I}lhan and {Feng}, Yu and {Moore}, Eric W. and {VanderPlas}, Jake and {Laxalde}, Denis and {Perktold}, Josef and {Cimrman}, Robert and {Henriksen}, Ian and {Quintero}, E.~A. and {Harris}, Charles R. and {Archibald}, Anne M. and {Ribeiro}, Ant{\^o}nio H. and {Pedregosa}, Fabian and {van Mulbregt}, Paul and {SciPy 1. 0 Contributors}},
        title = "{SciPy 1.0: fundamental algorithms for scientific computing in Python}",
      journal = {Nature Methods},
     keywords = {Computer Science - Mathematical Software, Computer Science - Data Structures and Algorithms, Computer Science - Software Engineering, Physics - Computational Physics},
         year = 2020,
        month = feb,
       volume = {17},
        pages = {261-272},
          doi = {10.1038/s41592-019-0686-2},
archivePrefix = {arXiv},
       eprint = {1907.10121},
 primaryClass = {cs.MS},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020NatMe..17..261V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sextractor.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{sextractor,
       author = {{Bertin}, E. and {Arnouts}, S.},
        title = "{SExtractor: Software for source extraction.}",
      journal = {A\&AS},
     keywords = {METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING, GALAXIES: PHOTOMETRY},
         year = 1996,
        month = jun,
       volume = {117},
        pages = {393-404},
          doi = {10.1051/aas:1996164},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&AS..117..393B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sip_tpv.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{sip-tpv,
   author = {{Shupe}, D.~L. and {Laher}, R.~R. and {Storrie-Lombardi}, L. and
	{Surace}, J. and {Grillmair}, C. and {Levitan}, D. and {Sesar}, B.
	},
    title = "{More flexibility in representing geometric distortion in astronomical images}",
     year = 2012,
   journal = {SPIE},
   volume = 8451,
    month = sep,
      eid = {84511M},
    pages = {84511M},
      doi = {10.1117/12.925460},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2012SPIE.8451E..1MS},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/swarp.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{swarp,
   author = {{Bertin}, E. and {Mellier}, Y. and {Radovich}, M. and {Missonnier}, G. and
    {Didelon}, P. and {Morin}, B.},
  journal = {ASPConf},
    title = "{The TERAPIX Pipeline}",
     year = {2002},
   volume = {281},
    pages = {228},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2002ASPC..281..228B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sympy.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@article{sympy,
 title = {SymPy: symbolic computing in Python},
 author = {Meurer, Aaron and Smith, Christopher P. and Paprocki, Mateusz and \v{C}ert\'{i}k, Ond\v{r}ej and Kirpichev, Sergey B. and Rocklin, Matthew and Kumar, AMiT and Ivanov, Sergiu and Moore, Jason K. and Singh, Sartaj and Rathnayake, Thilina and Vig, Sean and Granger, Brian E. and Muller, Richard P. and Bonazzi, Francesco and Gupta, Harsh and Vats, Shivam and Johansson, Fredrik and Pedregosa, Fabian and Curry, Matthew J. and Terrel, Andy R. and Rou\v{c}ka, \v{S}t\v{e}p\'{a}n and Saboo, Ashutosh and Fernando, Isuru and Kulal, Sumith and Cimrman, Robert and Scopatz, Anthony},
 year = 2017,
 month = jan,
 keywords = {Python, Computer algebra system, Symbolics},
 volume = 3,
 pages = {103},
 journal = {PeerJ CompSci},
 issn = {2376-5992},
 url = {https://doi.org/10.7717/peerj-cs.103},
 doi = {10.7717/peerj-cs.103}
}


==> reproduce/software/bibtex/tides.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{tides,
   author = {{Abad}, A. and {Barrio}, R. and {Belsa}, F. and {Rodriguez}, M},
    title = "{Algorithm 924: TIDES, a Taylor Series Integrator for Differential EquationS}",
  journal = {ACM TOMS},
     year = 2012,
    month = nov,
   volume = 39,
      eid = {5},
    pages = {1-28},
      doi = {10.1145/2382585.2382590},
 keywords = {Taylor series method, automatic differentiation, high precision, numerical integration of ODEs, variational equations},
}


==> reproduce/software/shell/git-post-checkout <==
#!@BINDIR@/bash
#
# The example hook script to store the metadata information of version
# controlled files (with each commit) using the 'metastore' program.
#
# Copyright (C) 2016 Przemyslaw Pawelczyk <przemoc@gmail.com>
# Copyright (C) 2018-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# This script is taken from the 'examples/hooks/pre-commit' file of the
# 'metastore' package (installed within the project, with an MIT license
# for copyright). We have just changed the name of the 'MSFILE' and also
# set special characters for the installation location of meta-store so our
# own installation is found by Git.
#
# Permission is hereby granted, free of charge, to any person obtaining a
# copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to permit
# persons to whom the Software is furnished to do so, subject to the
# following conditions:
#
# The above copyright notice and this permission notice shall be included
# in all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS
# OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN
# NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM,
# DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR
# OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE
# USE OR OTHER DEALINGS IN THE SOFTWARE.


# File containig the metadata and metastore executable.
MSFILE=".file-metadata"
MSBIN=@BINDIR@/metastore

# If metastore is not installed, then ignore this script (exit with a
# status of 0).
if [ ! -f $MSBIN ]; then exit 0; fi

# Delete all temporary files
find @TOP_PROJECT_DIR@/ -name "*~" -type f -delete

# Function to help in reporting a crash.
exit_on_fail() {
	"$@"
	if [ $? -ne 0 ]; then
		echo "Failed to execute: $@" >&2
		exit 1
	fi
}

# Check if the metadata file exists.
if [ ! -e "$MSFILE" ]; then
	echo "\"$MSFILE\" missing" >&2
	exit 1
fi

# Run metastore.
exit_on_fail \
       $MSBIN -a -m -e -E -q -O @USER@ -G @GROUP@ -f "$MSFILE"

# Return with a success code (0).
exit 0


==> reproduce/software/shell/git-pre-commit <==
#!@BINDIR@/bash
#
# The example hook script to store the metadata information of version
# controlled files (with each commit) using the 'metastore' program.
#
# Copyright (C) 2016 Przemyslaw Pawelczyk <przemoc@gmail.com>
# Copyright (C) 2018-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# WARNING:
#
# If the commit is aborted (e.g. by not entering any synopsis),
# then updated metastore file (.metadata by default) is not reverted,
# so its new version remains in the index.
# To undo any changes in metastore file written since HEAD commit,
# you may want to reset and checkout HEAD version of the file:
#
#     git reset HEAD -- .metadata
#     git checkout HEAD -- .metadata
#
# This script is taken from the 'examples/hooks/pre-commit' file of the
# 'metastore' package (installed within the project, with an MIT license
# for copyright). Here, the name of the 'MSFILE' and also set special
# characters for the installation location of meta-store so our own
# installation is found by Git.
#
# Permission is hereby granted, free of charge, to any person obtaining a
# copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to permit
# persons to whom the Software is furnished to do so, subject to the
# following conditions:
#
# The above copyright notice and this permission notice shall be included
# in all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS
# OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN
# NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM,
# DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR
# OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE
# USE OR OTHER DEALINGS IN THE SOFTWARE.

# File containig the metadata and metastore executable.
MSFILE=".file-metadata"
MSBIN=@BINDIR@/metastore

# If metastore is not installed, then ignore this script (exit with a
# status of 0).
if [ ! -f $MSBIN ]; then exit 0; fi

# Function to help in reporting a crash.
exit_on_fail() {
	"$@"
	if [ $? -ne 0 ]; then
		echo "Failed to execute: $@" >&2
		exit 1
	fi
}

# Run metastore.
exit_on_fail \
	$MSBIN -O @USER@ -G @GROUP@ -s -f "$MSFILE"

# If it's first metastore commit, store again to include $MSFILE in $MSFILE.
if ! git-ls-tree --name-only HEAD 2>/dev/null | grep -Fqx "$MSFILE"; then
	exit_on_fail \
	        $MSBIN -O @USER@ -G @GROUP@ -s -f "$MSFILE"
fi

# Check if the metadata file exists.
if [ ! -e "$MSFILE" ]; then
	echo "\"$MSFILE\" missing" >&2
	exit 1
fi

# Add the metadata file to the Git repository.
exit_on_fail \
	git-add "$MSFILE"

# Return with a success code (0).
exit 0


==> tex/build/macros/dependencies-bib.tex <==


@ARTICLE{gnuastro,
       author = {{Akhlaghi}, Mohammad and {Ichikawa}, Takashi},
        title = "{Noise-based Detection and Segmentation of Nebulous Objects}",
      journal = {ApJS},
     keywords = {galaxies: irregular, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = sep,
       volume = {220},
       number = {1},
          eid = {1},
        pages = {1},
          doi = {10.1088/0067-0049/220/1/1},
archivePrefix = {arXiv},
       eprint = {1505.01664},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..220....1A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> tex/src/preamble-maneage-default-style.tex <==
%% General paper's style settings.
%
%% This preamble can be completely ignored when including this TeX file in
%% another style. This is done because this LaTeX build is meant to be an
%% initial/internal phase or part of a larger effort, so it has a basic
%% style defined here as a preamble. To ignore it, uncomment or delete the
%% respective line in 'paper.tex'.
%
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%
%% This file is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the
%% Free Software Foundation, either version 3 of the License, or (at your
%% option) any later version.
%
%% This file is distributed in the hope that it will be useful, but WITHOUT
%% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General Public License
%% for more details.
%
%% You should have received a copy of the GNU General Public License along
%% with this file.  If not, see <http://www.gnu.org/licenses/>.





%% Font.
\usepackage[T1]{fontenc}
\usepackage{newtxtext}
\usepackage{newtxmath}





%% Print size
\usepackage[a4paper, includeheadfoot, body={18.7cm, 24.5cm}]{geometry}





%% Set the distance between the columns if two columns:
\setlength{\columnsep}{0.75cm}





% To allow figures to take up more space on the top of the page:
\renewcommand{\topfraction}{.99}
\renewcommand{\bottomfraction}{.7}
\renewcommand{\textfraction}{.05}
\renewcommand{\floatpagefraction}{.99}
\renewcommand{\dbltopfraction}{.99}
\renewcommand{\dblfloatpagefraction}{.99}
\setcounter{topnumber}{1}
\setcounter{bottomnumber}{0}
\setcounter{totalnumber}{2}
\setcounter{dbltopnumber}{1}





%% To make the footnotes align:
\usepackage[hang]{footmisc}
\setlength\footnotemargin{10pt}





%For including time in the title:
\usepackage{datetime}





%% Define the abstract environment
\renewenvironment{abstract}
 {\vspace{-0.5cm}\small%
  \list{}{%
    \setlength{\leftmargin}{2cm}%
    \setlength{\rightmargin}{\leftmargin}%
  }%
  \item\relax}
 {\endlist}





%% To keep the main page's code clean.
\newcommand{\includeabstract}[1]{%
\twocolumn[%
  \begin{@twocolumnfalse}%
    \maketitle%
    \begin{abstract}%
    #1%
    \end{abstract}%
    \vspace{1cm}%
  \end{@twocolumnfalse}%
  ]%
}





%% Basic header style
%% ------------------
%
%% The steps below are to use the necessary LaTeX packages to get the demo
%% Maneage paper running with a reasonably looking, custom paper style. If
%% you are using a custom journal style, feel free to delete these.

%% General page header settings.
\usepackage{fancyhdr}
\pagestyle{fancy}
\lhead{\footnotesize{\scshape Draft paper}, {\footnotesize nnn:i (pp), Year Month day}}
\rhead{\scshape\footnotesize YOUR-NAME et al.}
\cfoot{\thepage}
\setlength{\voffset}{0.75cm}
\setlength{\headsep}{0.2cm}
\setlength{\footskip}{0.75cm}
\renewcommand{\headrulewidth}{0pt}

%% Specific style for first page.
\fancypagestyle{firststyle}
{
  \lhead{\footnotesize{\scshape Draft paper}, nnn:i (pp), YYYY Month day\\
  \scriptsize \textcopyright YYYY, Your name. All rights reserved.}
  \rhead{\footnotesize \footnotesize \today, \currenttime\\}
}

%To set the style of the titles:
\usepackage{titlesec}
\titleformat{\section}
  {\centering\normalfont\uppercase}
  {\thesection.}
  {0em}
  { }
\titleformat{\subsection}
  {\centering\normalsize\slshape}
  {\thesubsection.}
  {0em}
  { }
\titleformat{\subsubsection}
  {\centering\small\slshape}
  {\thesubsubsection.}
  {0em}
  { }

%% Title and author information
\usepackage{authblk}
\renewcommand\Authfont{\small\scshape}
\renewcommand\Affilfont{\footnotesize\normalfont}
\setlength{\affilsep}{0.2cm}


==> tex/src/references.tex <==
%% Non-software BibTeX entries. The software-specific BibTeX entries are
%% stored in a '*.tex' file under the 'tex/dependencies' directory.
%
%% Copyright (C) 2018-2023 Mohammad Akhlaghi <mohammad:at:akhlaghi.org>
%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{lights,
       author = {{Trujillo}, Ignacio and {D'Onofrio}, Mauro and {Zaritsky}, Dennis and {Madrigal-Aguado}, Alberto and {Chamba}, Nushkia and {Golini}, Giulia and {Akhlaghi}, Mohammad and {Sharbaf}, Zahra and {Infante-Sainz}, Ra{\'u}l and {Rom{\'a}n}, Javier and {Morales-Socorro}, Carlos and {Sand}, David J. and {Martin}, Garreth},
        title = "{Introducing the LBT Imaging of Galactic Halos and Tidal Structures (LIGHTS) survey. A preview of the low surface brightness Universe to be unveiled by LSST}",
      journal = {\aap},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: halos, galaxies: photometry, galaxies: structure, dark matter, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = oct,
       volume = {654},
          eid = {A40},
        pages = {A40},
          doi = {10.1051/0004-6361/202141603},
archivePrefix = {arXiv},
       eprint = {2109.07478},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...654A..40T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{maneage,
       author = {{Akhlaghi}, Mohammad and {Infante-Sainz}, Raul and
         {Roukema}, Boudewijn F. and {Khellat}, Mohammadreza and
         {Valls-Gabaud}, David and {Baena-Galle}, Roberto},
        title = "{Toward Long-Term and Archivable Reproducibility}",
      journal = {CiSE},
     keywords = {Computer Science - Digital Libraries},
         year = 2021,
        month = may,
       volume = {23},
       number = {3},
        pages = {82-91},
          doi = {10.1109/MCSE.2021.3072860},
archivePrefix = {arXiv},
       eprint = {2006.03018},
 primaryClass = {cs.DL},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021CSE....23c..82A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{xdf,
       author = {{Illingworth}, G.~D. and {Magee}, D. and {Oesch}, P.~A. and {Bouwens}, R.~J. and {Labb{\'e}}, I. and {Stiavelli}, M. and {van Dokkum}, P.~G. and {Franx}, M. and {Trenti}, M. and {Carollo}, C.~M. and {Gonzalez}, V.},
        title = "{The HST eXtreme Deep Field (XDF): Combining All ACS and WFC3/IR Data on the HUDF Region into the Deepest Field Ever}",
      journal = {\apjs},
     keywords = {cosmology: observations, galaxies: abundances, galaxies: high-redshift, techniques: image processing, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = nov,
       volume = {209},
       number = {1},
          eid = {6},
        pages = {6},
          doi = {10.1088/0067-0049/209/1/6},
archivePrefix = {arXiv},
       eprint = {1305.1931},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJS..209....6I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{wcscelestial,
       author = {{Calabretta}, M.~R. and {Greisen}, E.~W.},
        title = "{Representations of celestial coordinates in FITS}",
      journal = {\aap},
     keywords = {methods: data analysis, techniques: image processing, astronomical data bases: miscellaneous, astrometry, Astrophysics},
         year = 2002,
        month = dec,
       volume = {395},
        pages = {1077-1122},
          doi = {10.1051/0004-6361:20021327},
archivePrefix = {arXiv},
       eprint = {astro-ph/0207413},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002A&A...395.1077C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

